Experimental study of 13C({\alpha},n)16O reactions in the Majorana Demonstrator calibration data

Neutron captures and delayed decays of reaction products are common sources of backgrounds in ultra-rare event searches. In this work, we studied $^{13}$C($\alpha,n)^{16}$O reactions induced by $\alpha$-particles emitted within the calibration sources of the \textsc{Majorana Demonstrator}. These sources are thorium-based calibration standards enclosed in carbon-rich materials. The reaction rate was estimated by using the 6129-keV $\gamma$-rays emitted from the excited $^{16}$O states that are populated when the incoming $\alpha$-particles exceed the reaction Q-value. Thanks to the excellent energy performance of the \textsc{Demonstrator}'s germanium detectors, these characteristic photons can be clearly observed in the calibration data. Facilitated by \textsc{Geant4} simulations, a comparison between the observed 6129-keV photon rates and predictions by a TALYS-based software was performed. The measurements and predictions were found to be consistent, albeit with large statistical uncertainties. This agreement provides support for background projections from ($\alpha,n$)-reactions in future double-beta decay search efforts.

==> acknowledgments.tex <==
\section{\label{sec:ack} Acknowledgements}
This material is based upon work supported by the U.S.~Department of Energy, Office of Science, Office of Nuclear Physics under contract / award numbers DE-AC02-05CH11231, DE-AC05-00OR22725, DE-AC05-76RL0130, DE-FG02-97ER41020, DE-FG02-97ER41033, DE-FG02-97ER41041, DE-SC0012612, DE-SC0014445, DE-SC0018060, and LANLEM77/LANLEM78. We acknowledge support from the Particle Astrophysics Program and Nuclear Physics Program of the National Science Foundation through grant numbers MRI-0923142, PHY-1003399, PHY-1102292, PHY-1206314, PHY-1614611, PHY-1812409, PHY-1812356, and PHY-2111140. We gratefully acknowledge the support of the Laboratory Directed Research \& Development (LDRD) program at Lawrence Berkeley National Laboratory for this work. We gratefully acknowledge the support of the U.S.~Department of Energy through the Los Alamos National Laboratory LDRD Program and through the Pacific Northwest National Laboratory LDRD Program for this work.  We gratefully acknowledge the support of the South Dakota Board of Regents Competitive Research Grant. We acknowledge support from the Russian Foundation for Basic Research, grant No.~15-02-02919. We acknowledge the support of the Natural Sciences and Engineering Research Council of Canada, funding reference number SAPIN-2017-00023, and from the Canada Foundation for Innovation John R.~Evans Leaders Fund.  This research used resources provided by the Oak Ridge Leadership Computing Facility at Oak Ridge National Laboratory and by the National Energy Research Scientific Computing Center, a U.S.~Department of Energy Office of Science User Facility. We thank our hosts and colleagues at the Sanford Underground Research Facility for their support.
